DIDChain: Advancing Supply Chain Data Management with Decentralized Identifiers and Blockchain

Supply chain data management faces challenges in traceability, transparency, and trust. These issues stem from data silos and communication barriers. This research introduces DIDChain, a framework leveraging blockchain technology, Decentralized Identifiers, and the InterPlanetary File System. DIDChain improves supply chain data management. To address privacy concerns, DIDChain employs a hybrid blockchain architecture that combines public blockchain transparency with the control of private systems. Our hybrid approach preserves the authenticity and reliability of supply chain events. It also respects the data privacy requirements of the participants in the supply chain. Central to DIDChain is the cheqd infrastructure. The cheqd infrastructure enables digital tracing of asset events, such as an asset moving from the milk-producing dairy farm to the cheese manufacturer. In this research, assets are raw materials and products. The cheqd infrastructure ensures the traceability and reliability of assets in the management of supply chain data. Our contribution to blockchain-enabled supply chain systems demonstrates the robustness of DIDChain. Integrating blockchain technology through DIDChain offers a solution to data silos and communication barriers. With DIDChain, we propose a framework to transform the supply chain infrastructure across industries.

==> tables/stakeholder.tex <==
\begin{table}[ht]
\centering
\caption{Roles and actions of stakeholders in the supply chain. Creation of DIDs referes to creation of digital twins.}
\label{tab:stakeholder_roles}
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X}
\toprule
\textbf{Stakeholder} & \textbf{Role} & \textbf{Actions} & \textbf{Verification Process} \\
\midrule
Issuer (e.g., Raw Material Producer) & Create \& Register DID & Produce raw material & - \\
Holder (e.g., Manufacturer) & Create \& Link DID Document & Receive \& Process materials & Validate DID Docs with signatures, hashes \\
Verifier (e.g., Distributor) & Verify DID Documents' trace & Receive \& Process products & Verify DID Docs for product legitimacy \\
\bottomrule
\end{tabularx}
\end{table}


\begin{comment}
\begin{table}[ht]
\centering
\caption{Stakeholder Relations in the Supply Chain}
\label{tab:stakeholder_relations}
\begin{tabular}{ | m{2.5cm} | m{2.5cm} | m{2.5cm} | m{2.5cm} | }
\hline
\textbf{Stakeholder} & \textbf{Role} & \textbf{Actions} & \textbf{Verification Process} \\
\hline
Issuer (e.g., Raw Material Producer) & Creating DID \& Register DID to blockchain& Producing raw material & -\\
\hline
Holder (e.g., Manufacturer) & Creating DID \& link DID Doc to containing raw materials & Receiving and processing raw material & DID Documents of raw materials are validated...TODO how? through blockchain for trusted issuer...\\
\hline
Verifier (e.g., Distributor) & Verify trace of DID Document of a product& Ensuring the material's and product's authenticity & DID Documents are verified to confirm the legitimacy of the product\\
\hline
\end{tabular}
\end{table}
\end{comment}

==> workingfolder/authors.tex <==
% Between 
% \title{DIDChain: Advancing Supply Chain Data Management with Decentralized Identifiers and Blockchain}
\begin{comment}
\author{\IEEEauthorblockN{\textbf{Anonymous Authors}}
\IEEEauthorblockA{\textit{} \\
\textit{}\\
}}
\end{comment}
% \author{\IEEEauthorblockN{\textbf{Anonymous Authors}}
% \IEEEauthorblockA{\textit{} \\
% \textit{}\\
% }}
% \maketitle

\begin{comment}
\author{\IEEEauthorblockN{Patrick Herbke \orcidlink{0000-0001-9649-2975}}
\IEEEauthorblockA{\textit{TU Berlin, Service-centric Networking}\\
Berlin, Germany \\
p.herbke@tu-berlin.de}
\and
\IEEEauthorblockN{Sid Lamichhane \orcidlink{0009-0000-5845-7060}}
\IEEEauthorblockA{\textit{TU Berlin, Service-centric Networking}\\
Berlin, Germany \\
lamichhane@tu-berlin.de}
\and
\IEEEauthorblockN{Kaustabh Barman \orcidlink{}}
\IEEEauthorblockA{\textit{TU Berlin, Service-centric Networking}\\
Berlin, Germany \\
kaustabh.barman@tu-berlin.de}
\and
\IEEEauthorblockN{Sanjeet Raj Pandey \orcidlink{0009-0007-9525-7587}}
\IEEEauthorblockA{\textit{TU Berlin, Service-centric Networking}\\
Berlin, Germany \\
s.pandey@tu-berlin.de}
\and
\IEEEauthorblockN{Axel K\"upper \orcidlink{0000-0002-4356-5613}}
\IEEEauthorblockA{\textit{TU Berlin, Service-centric Networking}\\
Berlin, Germany \\
axel.kuepper@tu-berlin.de}
\and
\IEEEauthorblockN{Andreas Abraham \orcidlink{0000-0002-4163-9113}}
\IEEEauthorblockA{\textit{ValidatedID S.L} \\
Barcelona, Spain \\
andreas.abraham@validatedid.com}
\and
\IEEEauthorblockN{Markus Sabadello \orcidlink{0000-0003-3603-0239}}
\IEEEauthorblockA{\textit{Danube Tech GmbH} \\
Vienna, Austria \\
markus@danubetech.com}
}
\end{comment}


%\begin{comment}
\author{\IEEEauthorblockN{
Patrick Herbke \orcidlink{0000-0001-9649-2975}\IEEEauthorrefmark{1}, 
Sid Lamichhane \orcidlink{0009-0000-5845-7060}\IEEEauthorrefmark{1}, 
Kaustabh Barman \orcidlink{0009-0001-9782-8917}\IEEEauthorrefmark{1}, 
Sanjeet Raj Pandey \orcidlink{0009-0007-9525-7587}\IEEEauthorrefmark{1}, 
Axel K\"upper \orcidlink{0000-0002-4356-5613}\IEEEauthorrefmark{1} \\ 
Andreas Abraham \orcidlink{0000-0002-4163-9113}\IEEEauthorrefmark{2}, 
Markus Sabadello \orcidlink{0000-0003-3603-0239}\IEEEauthorrefmark{3}
}
\IEEEauthorblockA{\IEEEauthorrefmark{1}Service-centric Networking,
Technische Universit\"at Berlin, Berlin, Germany\\
\{p.herbke, lamichhane, kaustabh.barman, s.pandey, axel.kuepper\}@tu-berlin.de}
\IEEEauthorblockA{\IEEEauthorrefmark{2}ValidatedID S.L, Barcelona, Spain, 
andreas.abraham@validatedid.com}
\IEEEauthorblockA{\IEEEauthorrefmark{3}Danube Tech GmbH, Vienna, Austria, 
markus@danubetech.com}}
%\end{comment}

% Contribution: PH 65%, Sid 23%, KB 2%, SR 1%, AK 3%, AA 3%, MS 3%

==> workingfolder/todo.tex <==
Given the detailed requirements and the need to integrate the discussion on revocation mechanisms for both DIDs and NFTs, as well as the authorization of issuers using OIDC-VC and its implementation with smart contracts, here's a streamlined to-do list for your IEEE conference paper on blockchain-based supply chain management. This list is designed to ensure that your paper is comprehensive, well-structured, and ready for submission to the IEEE conference.

####   0. Include Figures for: 
    - Supply Chain process (exemplarly with producing cheese) Asking Emanuele for co-authorship
    - Architecture: Where are the components located? On the computer? components description of function of the ccomponent...Frontend - User Interface (Website, React.js)
    
### Streamlined To-Do List

####   1. Introduction and Background
- * Enhancement Tip: Incorporate real-world statistics to emphasize the critical role of supply chain management and the impact of blockchain technology. Reference IEEE papers that have discussed the challenges in traditional supply chain systems and the potential of blockchain to address these challenges.
- **Complete the Introduction**: Emphasize the global importance of supply chain management, the challenges posed by traditional systems, and the potential of blockchain technology to address these challenges. Highlight the four Ts (traceability, transparency, tracking, and trust) and their relevance to supply chain management.
- **Expand the Background**:
  - **DIDs**: Provide a detailed explanation of Decentralized Identifiers (DIDs), their role in digital identity verification, and their importance in supply chain management. Include examples of DID documents and their history.
  - **Blockchain**: Describe the role of blockchain in ensuring traceability, transparency, and the integrity of transactions in global trade. Discuss the scalability challenges and how they are addressed by integrating IPFS.
  - **IPFS**: Explain the Interplanetary File System (IPFS) and its role in addressing scalability and data access challenges in blockchain technology.
  - **ERC721 NFTs**: Introduce ERC721 NFTs as a parallel development in the background, discussing their role in digital asset representation and their potential in supply chain management.

####   2. Conceptual Framework
- * Detailing the Framework: Ensure to cite sources from IEEE journals that have discussed the integration of blockchain, DIDs, and IPFS in similar contexts. This will not only strengthen your argument but also align your paper with IEEE standards.
Operational Mechanism: For each phase (DID Creation, Asset Registration, etc.), include examples or case studies from existing IEEE publications where similar approaches have been applied. This will provide a solid foundation for your proposed framework.
- **Detail the Conceptual Framework**: Elaborate on the integration of blockchain, DIDs, and IPFS for enhancing supply chain management. Describe how each technology contributes to the framework's objectives.
- **Explain the Operational Mechanism**:
  - **DID Creation and Asset Registration**: Describe the process of creating DIDs for assets and registering them with the issuer.
  - **DID Controller Ownership Change**: Explain how the DID controller's ownership changes during shipping and manufacturing events.
  - **Trace Verification Processes**: Detail the mechanisms for verifying the traceability of assets throughout the supply chain.
  - **ERC721 NFTs**: Discuss the conceptual framework for using ERC721 NFTs in parallel with DIDs for asset representation and verification.

####   3. Implementation
- * Technical Stack Description: When detailing the technical stack, compare your choices (React.js, Node.js, Cheqd, IPFS) with other alternatives by citing IEEE papers that have used different technologies. This comparison will demonstrate the rationale behind your technology selection.
Blockchain and Smart Contract Integration: Discuss the specific advantages of using Ethereum smart contracts in supply chain management, citing IEEE papers that have explored similar implementations. Highlight any unique aspects of your approach.
- **Describe the Implementation**: Outline the technical implementation of the framework, including the use of React.js, Express.js, Node.js, and the integration of Cheqd and IPFS.
- **Include Implementation Details**:
  - **APIs**: Discuss the APIs used for interacting with the blockchain and digital identities.
  - **Data Layer**: Explain how the data layer, underpinned by Cheqd and IPFS, ensures secure, decentralized storage and retrieval of supply chain information.
  - **ERC721 NFTs**: Describe the implementation of ERC721 NFTs for asset representation, including the creation, transfer, and verification of NFTs in the supply chain context.

Structure.
To create a robust Implementation section for your paper, you should address the following key aspects, considering the stringent standards of IEEE and ACM publications:

### 3. Implementation

1. **Layered Framework Design**:
   - Detail the multi-tiered architecture of your framework, emphasizing how each layer contributes to the overall functionality.
   - Explain the role of the front end, powered by React.js, in providing a dynamic user interface, citing relevant literature on the effectiveness of React.js in similar systems.

2. **Backend Technologies**:
   - Discuss the choice of Express.js and Node.js for backend services, providing comparisons with other backend technologies and justifying your choices based on performance, scalability, or other criteria.
   - Illustrate the backend's role in API communications and server-side functionalities.

3. **Blockchain and DID Resolver**:
   - Describe how the DID resolver functions within your API layer to connect blockchain and digital identities.
   - Provide technical details on the implementation of blockchain technology, focusing on how it enhances traceability and integrity in supply chain management.
   - Cite studies that discuss the integration of blockchain in supply chain systems to validate your approach.

4. **Credential Services and Web3 APIs**:
   - Elaborate on the authentication processes using Web3 APIs and credential services, including examples of interactions that occur during the supply chain process.
   - Support your discussion with references to ACM/IEEE papers that have explored the use of Web3 technologies in similar contexts.

5. **Data Layer and Decentralized Storage**:
   - Examine the implementation of IPFS for decentralized data storage, and its impact on data availability and system resilience.
   - Discuss the Cheqd blockchain's specific role in the data layer and how it differs from or improves upon traditional blockchain solutions in supply chain applications.

6. **Security and Decentralization**:
   - Address the security measures implemented to protect the integrity of supply chain data.
   - Explore the decentralization aspect of the framework, discussing its advantages in creating a resilient supply chain network.

7. **System Integration and Testing**:
   - Detail the process of integrating the various components of your framework, including challenges faced and how they were overcome.
   - Describe the testing methodologies used to ensure the reliability and performance of the system, referencing ACM/IEEE standards for software testing.

--- Info for Implementation ---

8. **Figure Explanations**:
   - Refer to figures that visually represent the architecture and data flow within your system, ensuring they are described in detail within the text.
   - Include diagrams that map out the API interactions and the flow of data between different system components.

9. **Evaluation of Economic Feasibility**:
   - Discuss the cost-effectiveness of your implementation, comparing it to traditional supply chain management systems.
   - Provide a cost-benefit analysis, referencing IEEE/ACM economic models where appropriate.

By structuring your Implementation section around these aspects and grounding your discussion in the existing body of IEEE/ACM literature, you will not only demonstrate the technical viability of your framework but also its relevance and superiority to current systems. Always ensure that your claims are substantiated with empirical data or citations from credible sources (GoogleScholar paper >50 citations best case, computer science conferences.

--- Info for Implementation ---


####   4. Evaluation
- * Methodological Approach: Align your evaluation framework with standard practices in IEEE publications. Consider incorporating benchmarks or standards from IEEE papers that have conducted similar analyses.
Comparative Insights: Use IEEE articles as benchmarks for comparing your Cheqd-based and smart contract-based implementations. This will provide a credible basis for your analysis.
- **Performance Metrics**: Define and measure the performance metrics for both the Cheqd-based implementation and the smart contract-based implementation using ERC721 NFTs. Include latency, performance, and costs. (SID: also compare timestamping functionality of did and smart contract based implementation)
- **Comparative Analysis**: Conduct a comparative analysis of the two implementations, highlighting the differences in performance, scalability, interoperability, cost efficiency, and security and privacy.
\begin{comment}
In the conclusion of an evaluation section, especially within a scientific context, it's essential to succinctly encapsulate the core findings, their significance, and the broader impact of your research. The conclusion should include:

Summary of Key Findings: Concisely recapitulate the primary outcomes of your evaluation. Highlight how your framework improves upon existing solutions in terms of efficiency, security, and economic viability.

Contribution to the Field: Clearly state how your research advances the knowledge within the supply chain management and blockchain domains. Emphasize the novel aspects of your framework and its practical implications.

Addressing the Research Objectives: Reiterate how your findings respond to the initial research questions or objectives outlined at the beginning of your study. This ties the conclusion back to the introduction, providing a sense of closure.

Implications for Practice: Discuss the practical applications of your findings. How can practitioners in the field of supply chain management leverage your blockchain-integrated framework? What operational or economic benefits might they expect?

Limitations and Future Research Directions: While briefly mentioned in a previous section, reiterate any significant limitations that constrain the interpretation of your results. Suggest areas for future research that can build on your findings, proposing how subsequent studies might overcome these limitations or explore new questions.

Final Statement: End with a strong, impactful statement that leaves a lasting impression on the reader. This could be a reflection on the potential future of blockchain in supply chain management or a call to action for further research and exploration in this area.

A well-crafted conclusion reinforces the value of your research, encourages further scholarly inquiry, and demonstrates how your work contributes to advancing both theory and practice.
\end{comment}
- **Discussion on Key Management**: Compare the client secret mode and the "Credential service" mode for key management, discussing their pros and cons.
- **Smart Contract vs. DID Document Solution**:
  - **ERC721 and DID Standard**: Analyze the discussion between Sid and yourself regarding the use of ERC721 for smart contracts and the DID standard for DID document solutions. Discuss the implications of each approach on the scalability, interoperability, and security of the supply chain management system.
  - **Implementation Comparison**: Provide a detailed comparison of the two implementations, focusing on the ease of integration, the flexibility of the system, and the potential for scalability. Discuss the advantages and disadvantages of each approach, including the impact on the overall efficiency and effectiveness of the supply chain management system.

**Evaluation of Economic Feasibility**:
   - Discuss the cost-effectiveness of your implementation, comparing it to traditional supply chain management systems.
   - Provide a cost-benefit analysis, referencing IEEE/ACM economic models where appropriate.
   
####   5. Revocation Mechanisms
- *Discussion on Revocation: Cite IEEE papers that have explored revocation mechanisms in blockchain systems. This will contextualize your discussion within the broader IEEE community's work on the topic.
- **Revocation of DIDs**: Discuss the mechanisms for revoking DIDs, including the process for deactivating a DID and the implications for supply chain traceability. (SID: even after deactivation of DID all its versionm can still be resolved, hence tracibility is still possible even if DID deactivated. DID deactivation makes sense for situation when underlying item cannot be shipped AND received AND used for manufacturing (if a material). Consequently these cases are loss of item, irreparable damage, item is faulty, item fails standards and regulations etc.) 
- **Revocation of NFTs**: Explain the revocation mechanisms for ERC721 NFTs within the blockchain context, discussing the potential for revoking or invalidating NFTs in the supply chain.

####   6. Authorization of Issuers with OIDC-VC
- * Smart Contract Implementation: Reference IEEE papers that have discussed the use of OIDC-VC with smart contracts, especially in supply chain scenarios. This will showcase your approach's novelty and relevance.
- **Implementation with Smart Contracts**: Discuss how OIDC-VC can be implemented with smart contracts to authorize issuers in the supply chain. Explain the process for issuing, verifying, and revoking verifiable credentials using smart contracts.

####   7. Related Work
- * Exhaustive Literature Review: Ensure that your review of related work covers the latest and most relevant IEEE publications in the field of blockchain-based supply chain management. Highlight how your work addresses gaps not covered by these publications.
- **Review Existing Literature**: Conduct a thorough review of existing works on blockchain-based supply chain management, focusing on the integration of DIDs, the use of IPFS, and the application of ERC721 NFTs.
- **Identify Gaps**: Identify gaps in the existing literature and how your research addresses these gaps.

####   8. Conclusion and Future Work
- *Summarization: Concisely summarize the key findings of your work, referencing IEEE standards for conclusions. Discuss the implications of your findings for future research, citing areas identified by IEEE publications as needing further exploration.
- **Summarize Findings**: Synthesize the findings of your research, discussing the implications for supply chain management and the broader field of blockchain technology.
- **Outline Future Research**: Suggest directions for future research, including potential improvements to the framework and new applications of blockchain, DIDs, and IPFS in supply chain management.

--- General Tips ---

####   9. Technical Details and Implementation
- **Finalize the LaTeX Code**: Ensure that all technical details, including code snippets and figures, are accurately represented in the LaTeX document.
- **Review and Optimize**: Conduct a thorough review of the paper, optimizing the text and structure for clarity and coherence.

####   10. Final Preparations
- **Proofread**: Perform a final proofreading to ensure the paper is free of errors and adheres to the IEEE style guide.
- **Prepare for Submission**: Compile the paper, ensuring all sections are complete and the document is ready for submission to the IEEE conference.

This streamlined to-do list is designed to guide you through the process of completing your paper, ensuring that it addresses the critical questions and requirements of the reviewers in your field. Each step is crucial for ensuring the paper is comprehensive, well-structured, and ready for submission to the IEEE conference.
